Abstract Syntax Networks for Code Generation and Semantic Parsing

Tasks like code generation and semantic parsing require mapping unstructured (or partially structured) inputs to well-formed, executable outputs. We introduce abstract syntax networks, a modeling framework for these problems. The outputs are represented as abstract syntax trees (ASTs) and constructed by a decoder with a dynamically-determined modular structure paralleling the structure of the output tree. On the benchmark Hearthstone dataset for code generation, our model obtains 79.2 BLEU and 22.7% exact match accuracy, compared to previous state-of-the-art values of 67.1 and 6.1%. Furthermore, we perform competitively on the Atis, Jobs, and Geo semantic parsing datasets with no task-specific engineering.

==> Makefile <==
TEXFLAGS = -e '$$pdflatex=q/pdflatex %O -shell-escape %S/' -pdf
LATEXMK = latexmk

PACKAGE = minted.dtx \
		  minted.ins \
		  minted.pdf \
		  README \
		  Makefile

.PHONY: minted all doc dist clean cleanall

minted: minted.sty

doc: minted.pdf

all: minted doc

minted.sty: minted.ins minted.dtx
	tex minted.ins

minted.pdf: minted.sty minted.gls minted.dtx
	$(LATEXMK) $(TEXFLAGS) minted.dtx

minted.gls: minted.glo
	makeindex -s gglo.ist -o minted.gls minted.glo

minted.glo: minted.dtx minted.sty
	$(LATEXMK) $(TEXFLAGS) minted.dtx

dist: $(PACKAGE)
	@$(RM) minted.zip
	@zip minted-$(shell grep '^\\ProvidesPackage' < minted.sty | grep -o '\<v[[:digit:]]*\.[[:digit:]]*\>').zip $(PACKAGE)

clean:
	@$(RM) *.aux *.log *.out *.toc *.fdb_latexmk *.ilg *.glo *.gls *.lol

cleanall: clean
	@$(RM) minted.sty minted.zip

